Holography Inspired Stringy Hadrons

Holography inspired stringy hadrons (HISH) is a set of models that describe hadrons: mesons, baryons and glueballs as strings in four dimensional space time. The models are based on a "map" from stringy hadrons of holographic confining backgrounds. In this note we review the "derivation" of the models. We start with a brief reminder of the passage from the AdS5xS5 string theory to certain flavored confining holographic models. We then describe the string configurations in holographic backgrounds that correspond to a Wilson line,a meson,a baryon and a glueball. The key ingredients of the four dimensional picture of hadrons are the "string endpoint mass" and the "baryonic string vertex". We determine the classical trajectories of the HISH. We review the current understanding of the quantization of the hadronic strings. We end with a summary of the comparison of the outcome of the HISH models with the PDG data about mesons and baryons. We extract the values of the tension, masses and intercepts from best fits, write down certain predictions for higher excited hadrons and present attempts to identify glueballs

==> HolStringyhadrons.tex <==
\providecommand{\href}[2]{#2}\begingroup\raggedright
\begin{thebibliography}{10}

\bibitem{Collins:book}
P.~Collins, {\it {An Introduction to Regge Theory and High Energy Physics}},
  {\em Cambridge Univeristy Press} (1977) 456.

\bibitem{Sonnenschein:2014jwa}
J.~Sonnenschein and D.~Weissman, {\it {Rotating strings confronting PDG
  mesons}},  {\em JHEP} {\bf 1408} (2014) 013,
  [\href{http://xxx.lanl.gov/abs/1402.5603}{{\tt arXiv:1402.5603}}].

\bibitem{Sonnenschein:2014bia}
J.~Sonnenschein and D.~Weissman, {\it {A rotating string model versus baryon
  spectra}},  {\em JHEP} {\bf 1502} (2015) 147,
  [\href{http://xxx.lanl.gov/abs/1408.0763}{{\tt arXiv:1408.0763}}].

%\cite{Sonnenschein:2015zaa}
\bibitem{Sonnenschein:2015zaa}
  J.~Sonnenschein and D.~Weissman,
  {\it{``Glueballs as rotating folded closed strings}}
  JHEP {\bf 1512}, 011 (2015)
  doi:10.1007/JHEP12(2015)011
  [arXiv:1507.01604 [hep-ph]].
  %%CITATION = doi:10.1007/JHEP12(2015)011;%%
  %3 citations counted in INSPIRE as of 15 Jan 2016



\bibitem{Baker:2002km}
M.~Baker and R.~Steinke, {\it {Semiclassical quantization of effective string
  theory and Regge trajectories}},  {\em Phys.Rev.} {\bf D65} (2002) 094042,
  [\href{http://xxx.lanl.gov/abs/hep-th/0201169}{{\tt hep-th/0201169}}].

\bibitem{Schreiber:2004ie}
E.~Schreiber, {\it {Excited mesons and quantization of string endpoints}},
  \href{http://xxx.lanl.gov/abs/hep-th/0403226}{{\tt hep-th/0403226}}.

\bibitem{Zahn:2013yma}
J.~Zahn, {\it {The excitation spectrum of rotating strings with masses at the
  ends}},  {\em JHEP} {\bf 1312} (2013) 047,
  [\href{http://xxx.lanl.gov/abs/1310.0253}{{\tt arXiv:1310.0253}}].

\bibitem{Hellerman:2013kba}
S.~Hellerman and I.~Swanson, {\it {String Theory of the Regge Intercept}},
  \href{http://xxx.lanl.gov/abs/1312.0999}{{\tt arXiv:1312.0999}}.

\bibitem{Aharony:2013ipa}
O.~Aharony and Z.~Komargodski, {\it {The Effective Theory of Long Strings}},
  {\em JHEP} {\bf 1305} (2013) 118,
  [\href{http://xxx.lanl.gov/abs/1302.6257}{{\tt arXiv:1302.6257}}].

%\cite{Erdmenger:2007cm}
\bibitem{Erdmenger:2007cm}
  J.~Erdmenger, N.~Evans, I.~Kirsch and E.~Threlfall,
  ``Mesons in Gauge/Gravity Duals - A Review,''
  Eur.\ Phys.\ J.\ A {\bf 35} (2008) 81
  doi:10.1140/epja/i2007-10540-1
  [arXiv:0711.4467 [hep-th]].
  %%CITATION = doi:10.1140/epja/i2007-10540-1;%%

\bibitem{Witten:1998zw}
E.~Witten, {\it {Anti-de Sitter space, thermal phase transition, and
  confinement in gauge theories}},  {\em Adv.Theor.Math.Phys.} {\bf 2} (1998)
  505--532, [\href{http://xxx.lanl.gov/abs/hep-th/9803131}{{\tt
  hep-th/9803131}}].

%\cite{Maldacena:1998im}
\bibitem{Maldacena:1998im}
  J.~M.~Maldacena,
  ``Wilson loops in large N field theories,''
  Phys.\ Rev.\ Lett.\  {\bf 80}, 4859 (1998)
  doi:10.1103/PhysRevLett.80.4859
  [hep-th/9803002].
  %%CITATION = doi:10.1103/PhysRevLett.80.4859;%%
  %1302 citations counted in INSPIRE as of 17 Jan 2016

%\cite{Polchinski:2000uf}
\bibitem{Polchinski:2000uf}
  J.~Polchinski and M.~J.~Strassler,
  ``The String dual of a confining four-dimensional gauge theory,''
  hep-th/0003136.
  %%CITATION = HEP-TH/0003136;%%
  %543 citations counted in INSPIRE as of 18 Jan 2016

%\cite{Aharony:2002up}
\bibitem{Aharony:2002up}
  O.~Aharony,
  ``The NonAdS / nonCFT correspondence, or three different paths to QCD,''
  hep-th/0212193.
  %%CITATION = HEP-TH/0212193;%%
  %64 citations counted in INSPIRE as of 18 Jan 2016

%\cite{Maldacena:2000yy}
\bibitem{Maldacena:2000yy}
  J.~M.~Maldacena and C.~Nunez,
  ``Towards the large N limit of pure N=1 superYang-Mills,''
  Phys.\ Rev.\ Lett.\  {\bf 86}, 588 (2001)
  doi:10.1103/PhysRevLett.86.588
  [hep-th/0008001].
  %%CITATION = doi:10.1103/PhysRevLett.86.588;%%
  %602 citations counted in INSPIRE as of 18 Jan 2016

%\cite{Polchinski:2002jw}
\bibitem{Polchinski:2002jw}
  J.~Polchinski and M.~J.~Strassler,
  ``Deep inelastic scattering and gauge / string duality,''
  JHEP {\bf 0305}, 012 (2003)
  doi:10.1088/1126-6708/2003/05/012
  [hep-th/0209211].
  %%CITATION = doi:10.1088/1126-6708/2003/05/012;%%
  %327 citations counted in INSPIRE as of 19 Jan 2016
%\cite{Klebanov:2000hb}
\bibitem{Klebanov:2000hb}
  I.~R.~Klebanov and M.~J.~Strassler,
  ``Supergravity and a confining gauge theory: Duality cascades and chi SB resolution of naked singularities,''
  JHEP {\bf 0008}, 052 (2000)
  doi:10.1088/1126-6708/2000/08/052
  [hep-th/0007191].
  %%CITATION = doi:10.1088/1126-6708/2000/08/052;%%
  %1410 citations counted in INSPIRE as of 19 janv. 2016

  %\cite{Gursoy:2007cb}
\bibitem{Gursoy:2007cb}
  U.~Gursoy and E.~Kiritsis,
  ``Exploring improved holographic theories for QCD: Part I,''
  JHEP {\bf 0802}, 032 (2008)
  doi:10.1088/1126-6708/2008/02/032
  [arXiv:0707.1324 [hep-th]].
  %%CITATION = doi:10.1088/1126-6708/2008/02/032;%%
  %234 citations counted in INSPIRE as of 19 janv. 2016



%\cite{Itzhaki:1998dd}
\bibitem{Itzhaki:1998dd}
  N.~Itzhaki, J.~M.~Maldacena, J.~Sonnenschein and S.~Yankielowicz,
  ``Supergravity and the large N limit of theories with sixteen supercharges,''
  Phys.\ Rev.\ D {\bf 58}, 046004 (1998)
  doi:10.1103/PhysRevD.58.046004
  [hep-th/9802042].
  %%CITATION = doi:10.1103/PhysRevD.58.046004;%%
  %791 citations counted in INSPIRE as of 19 Jan 2016

\bibitem{Kuperstein:2004yf}
S.~Kuperstein and J.~Sonnenschein, {\it {Non-critical, near extremal AdS(6)
  background as a holographic laboratory of four dimensional YM theory}},  {\em
  JHEP} {\bf 0411} (2004) 026,
  [\href{http://xxx.lanl.gov/abs/hep-th/0411009}{{\tt hep-th/0411009}}].

%\cite{Karch:2002sh}
\bibitem{Karch:2002sh}
  A.~Karch and E.~Katz,
  ``Adding flavor to AdS / CFT,''
  JHEP {\bf 0206}, 043 (2002)
  doi:10.1088/1126-6708/2002/06/043
  [hep-th/0205236].
  %%CITATION = doi:10.1088/1126-6708/2002/06/043;%%
  %771 citations counted in INSPIRE as of 19 janv. 2016
%\cite{Kruczenski:2003be}
\bibitem{Kruczenski:2003be}
  M.~Kruczenski, D.~Mateos, R.~C.~Myers and D.~J.~Winters,
  ``Meson spectroscopy in AdS / CFT with flavor,''
  JHEP {\bf 0307} (2003) 049
  doi:10.1088/1126-6708/2003/07/049
  [hep-th/0304032].
  %%CITATION = doi:10.1088/1126-6708/2003/07/049;%%
  %424 citations counted in INSPIRE as of 19 janv. 2016


  %325 citations counted in INSPIRE as of 19 Jan 2016

%\cite{Burrington:2004id}
\bibitem{Burrington:2004id}
  B.~A.~Burrington, J.~T.~Liu, L.~A.~Pando Zayas and D.~Vaman,
  ``Holographic duals of flavored N=1 super Yang-mills: Beyond the probe approximation,''
  JHEP {\bf 0502}, 022 (2005)
  doi:10.1088/1126-6708/2005/02/022
  [hep-th/0406207].
  %%CITATION = doi:10.1088/1126-6708/2005/02/022;%%
  %89 citations counted in INSPIRE as of 19 janv. 2016
%\cite{Sakai:2003wu}
\bibitem{Sakai:2003wu}
  T.~Sakai and J.~Sonnenschein,
  ``Probing flavored mesons of confining gauge theories by supergravity,''
  JHEP {\bf 0309}, 047 (2003)
  doi:10.1088/1126-6708/2003/09/047
  [hep-th/0305049].
  %%CITATION = doi:10.1088/1126-6708/2003/09/047;%%
  %124 citations counted in INSPIRE as of 19 janv. 2016

  %\cite{Jarvinen:2011qe}
\bibitem{Jarvinen:2011qe}
  M.~Jarvinen and E.~Kiritsis,
  ``Holographic Models for QCD in the Veneziano Limit,''
  JHEP {\bf 1203}, 002 (2012)
  doi:10.1007/JHEP03(2012)002
  [arXiv:1112.1261 [hep-ph]].
  %%CITATION = doi:10.1007/JHEP03(2012)002;%%
  %56 citations counted in INSPIRE as of 19 janv. 2016





\bibitem{SakSug}
T.~Sakai and S.~Sugimoto, {\it {Low energy hadron physics in holographic QCD}},
   {\em Prog.Theor.Phys.} {\bf 113} (2005) 843--882,
  [\href{http://xxx.lanl.gov/abs/hep-th/0412141}{{\tt hep-th/0412141}}].

\bibitem{Casero:2005se}
R.~Casero, A.~Paredes, and J.~Sonnenschein, {\it {Fundamental matter, meson
  spectroscopy and non-critical string/gauge duality}},  {\em JHEP} {\bf 0601}
  (2006) 127, [\href{http://xxx.lanl.gov/abs/hep-th/0510110}{{\tt
  hep-th/0510110}}].

\bibitem{oai:arXiv.org:0806.0152}
O.~Mintakevich and J.~Sonnenschein, {\it {On the spectra of scalar mesons from
  HQCD models}},  {\em JHEP} {\bf 0808} (2008) 082,
  [\href{http://xxx.lanl.gov/abs/0806.0152}{{\tt arXiv:0806.0152}}].

\bibitem{Peeters:2006iu}
K.~Peeters, J.~Sonnenschein, and M.~Zamaklar, {\it {Holographic melting and
  related properties of mesons in a quark gluon plasma}},  {\em Phys.Rev.} {\bf
  D74} (2006) 106008, [\href{http://xxx.lanl.gov/abs/hep-th/0606195}{{\tt
  hep-th/0606195}}].

\bibitem{oai:arXiv.org:hep-ph/0602229}
A.~Karch, E.~Katz, D.~T. Son, and M.~A. Stephanov, {\it {Linear confinement and
  AdS/QCD}},  {\em Phys.Rev.} {\bf D74} (2006) 015005,
  [\href{http://xxx.lanl.gov/abs/hep-ph/0602229}{{\tt hep-ph/0602229}}].

\bibitem{Imoto:2010ef}
T.~Imoto, T.~Sakai, and S.~Sugimoto, {\it {Mesons as Open Strings in a
  Holographic Dual of QCD}},  {\em Prog.Theor.Phys.} {\bf 124} (2010) 263--284,
  [\href{http://xxx.lanl.gov/abs/1005.0655}{{\tt arXiv:1005.0655}}].

\bibitem{PandoZayas:2003yb}
L.~A. Pando~Zayas, J.~Sonnenschein, and D.~Vaman, {\it {Regge trajectories
  revisited in the gauge / string correspondence}},  {\em Nucl.Phys.} {\bf
  B682} (2004) 3--44, [\href{http://xxx.lanl.gov/abs/hep-th/0311190}{{\tt
  hep-th/0311190}}].



\bibitem{Kruczenski:2004me}
M.~Kruczenski, L.~A. Pando~Zayas, J.~Sonnenschein, and D.~Vaman, {\it {Regge
  trajectories for mesons in the holographic dual of large-N(c) QCD}},  {\em
  JHEP} {\bf 0506} (2005) 046,
  [\href{http://xxx.lanl.gov/abs/hep-th/0410035}{{\tt hep-th/0410035}}].

\bibitem{cobitalks}
J.~Sonnenschein, {\it Holographic stingy hadrons},  {\em Talks delivered in
  September IPMU, October NBI and November NS/WAS 2013}.

\bibitem{Peeters:2005fq}
K.~Peeters, J.~Sonnenschein, and M.~Zamaklar, {\it {Holographic decays of
  large-spin mesons}},  {\em JHEP} {\bf 0602} (2006) 009,
  [\href{http://xxx.lanl.gov/abs/hep-th/0511044}{{\tt hep-th/0511044}}].

\bibitem{oai:arXiv.org:hep-th/9911123}
Y.~Kinar, E.~Schreiber, J.~Sonnenschein, and N.~Weiss, {\it {Quantum
  fluctuations of Wilson loops from string models}},  {\em Nucl.Phys.} {\bf
  B583} (2000) 76--104, [\href{http://xxx.lanl.gov/abs/hep-th/9911123}{{\tt
  hep-th/9911123}}].


%\cite{Hellerman:2014cba}
\bibitem{Hellerman:2014cba}
  S.~Hellerman, S.~Maeda, J.~Maltz and I.~Swanson,
  ``Effective String Theory Simplified,''
  JHEP {\bf 1409}, 183 (2014)
  doi:10.1007/JHEP09(2014)183
  [arXiv:1405.6197 [hep-th]].
  %%CITATION = doi:10.1007/JHEP09(2014)183;%%
  %3 citations counted in INSPIRE as of 16 Jan 2016

\bibitem{Chodos:1973gt}
A.~Chodos and C.~B. Thorn, {\it {Making the Massless String Massive}},  {\em
  Nucl.Phys.} {\bf B72} (1974) 509.







\bibitem{Arvis:1983fp}
J.~Arvis, {\it {The Exact $q \bar{q}$ Potential in Nambu String Theory}},  {\em
  Phys.Lett.} {\bf B127} (1983) 106.



\bibitem{PDG:2012}
{\bf Particle Data Group} Collaboration, J.~Beringer et~al., {\it {Review of
  Particle Physics (RPP)}},  {\em Phys.Rev.} {\bf D86} (2012) 010001.

\bibitem{Eichten:2007qx}
E.~Eichten, S.~Godfrey, H.~Mahlke, and J.~L. Rosner, {\it {Quarkonia and their
  transitions}},  {\em Rev.Mod.Phys.} {\bf 80} (2008) 1161--1193,
  [\href{http://xxx.lanl.gov/abs/hep-ph/0701208}{{\tt hep-ph/0701208}}].

\bibitem{Brambilla:2010cs}
N.~Brambilla, S.~Eidelman, B.~Heltsley, R.~Vogt, G.~Bodwin, et~al., {\it {Heavy
  quarkonium: progress, puzzles, and opportunities}},  {\em Eur.Phys.J.} {\bf
  C71} (2011) 1534, [\href{http://xxx.lanl.gov/abs/1010.5827}{{\tt
  arXiv:1010.5827}}].

\bibitem{Anisovich:2000kxa}
A.~Anisovich, V.~Anisovich, and A.~Sarantsev, {\it {Systematics of q anti-q
  states in the (n, M**2) and (J, M**2) planes}},  {\em Phys.Rev.} {\bf D62}
  (2000) 051502, [\href{http://xxx.lanl.gov/abs/hep-ph/0003113}{{\tt
  hep-ph/0003113}}].

\bibitem{Gershtein:2006ng}
S.~Gershtein, A.~Likhoded, and A.~a. Luchinsky, {\it {Systematics of heavy
  quarkonia from Regge trajectories on (n,M**2) and (M**2,J) planes}},  {\em
  Phys.Rev.} {\bf D74} (2006) 016002,
  [\href{http://xxx.lanl.gov/abs/hep-ph/0602048}{{\tt hep-ph/0602048}}].

\bibitem{Ebert:2009ub}
D.~Ebert, R.~Faustov, and V.~Galkin, {\it {Mass spectra and Regge trajectories
  of light mesons in the relativistic quark model}},  {\em Phys.Rev.} {\bf D79}
  (2009) 114029, [\href{http://xxx.lanl.gov/abs/0903.5183}{{\tt
  arXiv:0903.5183}}].

\bibitem{Ebert:2009ua}
D.~Ebert, R.~Faustov, and V.~Galkin, {\it {Heavy-light meson spectroscopy and
  Regge trajectories in the relativistic quark model}},  {\em Eur.Phys.J.} {\bf
  C66} (2010) 197--206, [\href{http://xxx.lanl.gov/abs/0910.5612}{{\tt
  arXiv:0910.5612}}].

\bibitem{Ebert:2011jc}
D.~Ebert, R.~Faustov, and V.~Galkin, {\it {Spectroscopy and Regge trajectories
  of heavy quarkonia and $B_c$ mesons}},  {\em Eur.Phys.J.} {\bf C71} (2011)
  1825, [\href{http://xxx.lanl.gov/abs/1111.0454}{{\tt arXiv:1111.0454}}].

\bibitem{Aaij:2013sza}
{\bf LHCb} Collaboration, R.~Aaij et~al., {\it {Study of $D_J$ meson decays to
  $D^+\pi^-$, $D^0 \pi^+$ and $D^{*+}\pi^-$ final states in pp collision}},
  {\em JHEP} {\bf 1309} (2013) 145,
  [\href{http://xxx.lanl.gov/abs/1307.4556}{{\tt arXiv:1307.4556}}].

\bibitem{Wang:2013tka}
Z.-G. Wang, {\it {Analysis of strong decays of the charmed mesons $D_J(2580)$,
  $D_J^*(2650)$, $D_J(2740)$, $D^*_J(2760)$, $D_J(3000)$, $D_J^*(3000)$}},
  {\em Phys.Rev.} {\bf D88} (2013) 114003,
  [\href{http://xxx.lanl.gov/abs/1308.0533}{{\tt arXiv:1308.0533}}].


 %\cite{Kol:2010fq}
\bibitem{Kol:2010fq}
  U.~Kol and J.~Sonnenschein,
  %``Can holography reproduce the QCD Wilson line?,''
  JHEP {\bf 1105}, 111 (2011)
  doi:10.1007/JHEP05(2011)111
  [arXiv:1012.5974 [hep-th]].
  %%CITATION = doi:10.1007/JHEP05(2011)111;%%
  %11 citations counted in INSPIRE as of 28 Nov 2015

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\providecommand{\href}[2]{#2}\begingroup\raggedright\begin{thebibliography}{10}

 
\bibitem{Inopin:1999nf}
A.~Inopin and G.~Sharov, {\it {Hadronic Regge trajectories: Problems and
  approaches}},  {\em Phys.Rev.} {\bf D63} (2001) 054023,
  [\href{http://xxx.lanl.gov/abs/hep-ph/9905499}{{\tt hep-ph/9905499}}].

\bibitem{Tang:2000tb}
A.~Tang and J.~W. Norbury, {\it {Properties of Regge trajectories}},  {\em
  Phys.Rev.} {\bf D62} (2000) 016006,
  [\href{http://xxx.lanl.gov/abs/hep-ph/0004078}{{\tt hep-ph/0004078}}].

\bibitem{Klempt:2009pi}
E.~Klempt and J.-M. Richard, {\it {Baryon spectroscopy}},  {\em Rev.Mod.Phys.}
  {\bf 82} (2010) 1095--1153, [\href{http://xxx.lanl.gov/abs/0901.2055}{{\tt
  arXiv:0901.2055}}].

\bibitem{Hata:2007mb}
H.~Hata, T.~Sakai, S.~Sugimoto, and S.~Yamato, {\it {Baryons from instantons in
  holographic QCD}},  {\em Prog.Theor.Phys.} {\bf 117} (2007) 1157,
  [\href{http://xxx.lanl.gov/abs/hep-th/0701280}{{\tt hep-th/0701280}}].

\bibitem{Kaplunovsky:2010eh}
V.~Kaplunovsky and J.~Sonnenschein, {\it {Searching for an Attractive Force in
  Holographic Nuclear Physics}},  {\em JHEP} {\bf 1105} (2011) 058,
  [\href{http://xxx.lanl.gov/abs/1003.2621}{{\tt arXiv:1003.2621}}].

\bibitem{Kaplunovsky:2012gb}
V.~Kaplunovsky, D.~Melnikov, and J.~Sonnenschein, {\it {Baryonic Popcorn}},
  {\em JHEP} {\bf 1211} (2012) 047,
  [\href{http://xxx.lanl.gov/abs/1201.1331}{{\tt arXiv:1201.1331}}].

\bibitem{Kaplunovsky:2013iza}
V.~Kaplunovsky and J.~Sonnenschein, {\it {Dimension Changing Phase Transitions
  in Instanton Crystals}},  {\em JHEP} {\bf 1404} (2014) 022,
  [\href{http://xxx.lanl.gov/abs/1304.7540}{{\tt arXiv:1304.7540}}].


%\cite{Burrington:2007qd}
\bibitem{Burrington:2007qd}
  B.~A.~Burrington, V.~S.~Kaplunovsky and J.~Sonnenschein,
  ``Localized Backreacted Flavor Branes in Holographic QCD,''
  JHEP {\bf 0802}, 001 (2008)
  doi:10.1088/1126-6708/2008/02/001
  [arXiv:0708.1234 [hep-th]].
  %%CITATION = doi:10.1088/1126-6708/2008/02/001;%%
  %41 citations counted in INSPIRE as of 17 Jan 2016
	
	%\cite{Aharony:2006da}
\bibitem{Aharony:2006da}
  O.~Aharony, J.~Sonnenschein and S.~Yankielowicz,
  %``A Holographic model of deconfinement and chiral symmetry restoration,''
  Annals Phys.\  {\bf 322}, 1420 (2007)
  doi:10.1016/j.aop.2006.11.002
  [hep-th/0604161].
  %%CITATION = doi:10.1016/j.aop.2006.11.002;%%
  %240 citations counted in INSPIRE as of 17 Jan 2016
	
	%\cite{Bergman:2007pm}
\bibitem{Bergman:2007pm}
  O.~Bergman, S.~Seki and J.~Sonnenschein,
  %``Quark mass and condensate in HQCD,''
  JHEP {\bf 0712}, 037 (2007)
  doi:10.1088/1126-6708/2007/12/037
  [arXiv:0708.2839 [hep-th]].
  %%CITATION = doi:10.1088/1126-6708/2007/12/037;%%
  %81 citations counted in INSPIRE as of 17 Jan 2016
	
	%\cite{Casero:2007ae}
\bibitem{Casero:2007ae}
  R.~Casero, E.~Kiritsis and A.~Paredes,
  ``Chiral symmetry breaking as open string tachyon condensation,''
  Nucl.\ Phys.\ B {\bf 787}, 98 (2007)
  doi:10.1016/j.nuclphysb.2007.07.009
  [hep-th/0702155 [HEP-TH]].
  %%CITATION = doi:10.1016/j.nuclphysb.2007.07.009;%%
  %124 citations counted in INSPIRE as of 17 Jan 2016
%\cite{Brandhuber:1998er}

%\cite{Dhar:2007bz}
\bibitem{Dhar:2007bz}
  A.~Dhar and P.~Nag,
  ``Sakai-Sugimoto model, Tachyon Condensation and Chiral symmetry Breaking,''
  JHEP {\bf 0801}, 055 (2008)
  doi:10.1088/1126-6708/2008/01/055
  [arXiv:0708.3233 [hep-th]].
  %%CITATION = doi:10.1088/1126-6708/2008/01/055;%%
  %72 citations counted in INSPIRE as of 17 Jan 2016
	%\cite{Aharony:2008an}
\bibitem{Aharony:2008an}
  O.~Aharony and D.~Kutasov,
  ``Holographic Duals of Long Open Strings,''
  Phys.\ Rev.\ D {\bf 78}, 026005 (2008)
  doi:10.1103/PhysRevD.78.026005
  [arXiv:0803.3547 [hep-th]].
  %%CITATION = doi:10.1103/PhysRevD.78.026005;%%
  %60 citations counted in INSPIRE as of 17 Jan 2016
	
\bibitem{Brandhuber:1998er}
  A.~Brandhuber, N.~Itzhaki, J.~Sonnenschein and S.~Yankielowicz,
  {\it{Wilson loops, confinement, and phase transitions in large N gauge theories from supergravity,}}
  JHEP {\bf 9806}, 001 (1998)
  doi:10.1088/1126-6708/1998/06/001
  [hep-th/9803263].
  %%CITATION = doi:10.1088/1126-6708/1998/06/001;%%
  %187 citations counted in INSPIRE as of 15 Jan 2016


\bibitem{Brandhuber:1998xy}
A.~Brandhuber, N.~Itzhaki, J.~Sonnenschein, and S.~Yankielowicz, {\it {Baryons
  from supergravity}},  {\em JHEP} {\bf 9807} (1998) 020,
  [\href{http://xxx.lanl.gov/abs/hep-th/9806158}{{\tt hep-th/9806158}}].

\bibitem{Callan:1999zf}
J.~Callan, Curtis~G., A.~Guijosa, K.~G. Savvidy, and O.~Tafjord, {\it {Baryons
  and flux tubes in confining gauge theories from brane actions}},  {\em
  Nucl.Phys.} {\bf B555} (1999) 183--200,
  [\href{http://xxx.lanl.gov/abs/hep-th/9902197}{{\tt hep-th/9902197}}].

\bibitem{Dymarsky:2009cm}
A.~Dymarsky, S.~Kuperstein, and J.~Sonnenschein, {\it {Chiral Symmetry Breaking
  with non-SUSY D7-branes in ISD backgrounds}},  {\em JHEP} {\bf 0908} (2009)
  005, [\href{http://xxx.lanl.gov/abs/0904.0988}{{\tt arXiv:0904.0988}}].

\bibitem{Seki:2008mu}
S.~Seki and J.~Sonnenschein, {\it {Comments on Baryons in Holographic QCD}},
  {\em JHEP} {\bf 0901} (2009) 053,
  [\href{http://xxx.lanl.gov/abs/0810.1633}{{\tt arXiv:0810.1633}}].

  

\bibitem{Witten:1998xy}
E.~Witten, {\it {Baryons and branes in anti-de Sitter space}},  {\em JHEP} {\bf
  9807} (1998) 006, [\href{http://xxx.lanl.gov/abs/hep-th/9805112}{{\tt
  hep-th/9805112}}].

\bibitem{Dymarsky:2010ci}
A.~Dymarsky, D.~Melnikov, and J.~Sonnenschein, {\it {Attractive Holographic
  Baryons}},  {\em JHEP} {\bf 1106} (2011) 145,
  [\href{http://xxx.lanl.gov/abs/1012.1616}{{\tt arXiv:1012.1616}}].

\bibitem{'tHooft:2004he}
G.~'t~Hooft, {\it {Minimal strings for baryons}},
  \href{http://xxx.lanl.gov/abs/hep-th/0408148}{{\tt hep-th/0408148}}.

\bibitem{Sharov:2000pg}
G.~Sharov, {\it {Quasirotational motions and stability problem in dynamics of
  string hadron models}},  {\em Phys.Rev.} {\bf D62} (2000) 094015,
  [\href{http://xxx.lanl.gov/abs/hep-ph/0004003}{{\tt hep-ph/0004003}}].

\bibitem{ThesisFederovsky}
E.~Federovsky, {\it {Stringy baryons and scattering amplitudes}},  Master's
  thesis, Tel Aviv University, August, 2010.

\bibitem{ThesisHarpaz}
G.~Harpaz, {\it {Simulating stringy baryons}},  Master's thesis, Tel Aviv
  University, June, 2008.

\bibitem{Sharov:2013tga}
G.~Sharov, {\it {String Models, Stability and Regge Trajectories for Hadron
  States}},  \href{http://xxx.lanl.gov/abs/1305.3985}{{\tt arXiv:1305.3985}}.

\bibitem{Selem:2006nd}
A.~Selem and F.~Wilczek, {\it {Hadron systematics and emergent diquarks}},
  \href{http://xxx.lanl.gov/abs/hep-ph/0602128}{{\tt hep-ph/0602128}}.

\bibitem{Friedmann:2014qpa}
T.~Friedmann, {\it {QCD vs. the Centrifugal Barrier: a New QCD Effect}},  {\em
  EPJ Web Conf.} {\bf 70} (2014) 00027.

\bibitem{Sharov:1998hi}
G.~Sharov, {\it {String baryon model 'triangle': Hypocycloidal solutions}},
  {\em Phys.Rev.} {\bf D58} (1998) 114009,
  [\href{http://xxx.lanl.gov/abs/hep-th/9808099}{{\tt hep-th/9808099}}].


\bibitem{Decays}
J.~Sonnenschein and D.~Weissman, {\it {On decays of stringy hadrons [work in
  progress]}}, .

%\end{thebibliography}\endgroup
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\bibitem{Csaki:1998qr}
C.~Csaki, H.~Ooguri, Y.~Oz, and J.~Terning, {\it {Glueball mass spectrum from
  supergravity}},  {\em JHEP} {\bf 9901} (1999) 017,
  [\href{http://xxx.lanl.gov/abs/hep-th/9806021}{{\tt hep-th/9806021}}].

\bibitem{Brower:2000rp}
R.~C. Brower, S.~D. Mathur, and C.-I. Tan, {\it {Glueball spectrum for QCD from
  AdS supergravity duality}},  {\em Nucl. Phys.} {\bf B587} (2000) 249--276,
  [\href{http://xxx.lanl.gov/abs/hep-th/0003115}{{\tt hep-th/0003115}}].

\bibitem{Elander:2013jqa}
D.~Elander, A.~F. Faedo, C.~Hoyos, D.~Mateos, and M.~Piai, {\it {Multiscale
  confining dynamics from holographic RG flows}},  {\em JHEP} {\bf 05} (2014)
  003, [\href{http://xxx.lanl.gov/abs/1312.7160}{{\tt arXiv:1312.7160}}].

\bibitem{Bhanot:1980fx}
G.~Bhanot and C.~Rebbi, {\it {SU(2) String Tension, Glueball Mass and
  Interquark Potential by Monte Carlo Computations}},  {\em Nucl.Phys.} {\bf
  B180} (1981) 469.

\bibitem{Niemi:2003hb}
A.~J. Niemi, {\it {Are glueballs knotted closed strings?}},
  \href{http://xxx.lanl.gov/abs/hep-th/0312133}{{\tt hep-th/0312133}}.

\bibitem{Sharov:2007ag}
G.~Sharov, {\it {Closed String with Masses in Models of Baryons and
  Glueballs}},  \href{http://xxx.lanl.gov/abs/0712.4052}{{\tt
  arXiv:0712.4052}}.

\bibitem{Solovev:2000nb}
L.~Solovev, {\it {Glueballs in the string quark model}},  {\em
  Theor.Math.Phys.} {\bf 126} (2001) 203--211,
  [\href{http://xxx.lanl.gov/abs/hep-ph/0006010}{{\tt hep-ph/0006010}}].

\bibitem{Talalov:2001cp}
S.~Talalov, {\it {The Glueball Regge trajectory from the string inspired
  theory}},  \href{http://xxx.lanl.gov/abs/hep-ph/0101028}{{\tt
  hep-ph/0101028}}.

\bibitem{LlanesEstrada:2000jw}
F.~J. Llanes-Estrada, S.~R. Cotanch, P.~J. de~A.~Bicudo, J.~E.~F. Ribeiro, and
  A.~P. Szczepaniak, {\it {QCD glueball Regge trajectories and the Pomeron}},
  {\em Nucl.Phys.} {\bf A710} (2002) 45--54,
  [\href{http://xxx.lanl.gov/abs/hep-ph/0008212}{{\tt hep-ph/0008212}}].

\bibitem{Szczepaniak:2003mr}
A.~P. Szczepaniak and E.~S. Swanson, {\it {The Low lying glueball spectrum}},
  {\em Phys.Lett.} {\bf B577} (2003) 61--66,
  [\href{http://xxx.lanl.gov/abs/hep-ph/0308268}{{\tt hep-ph/0308268}}].

\bibitem{Pons:2004dk}
J.~Pons, J.~Russo, and P.~Talavera, {\it {Semiclassical string spectrum in a
  string model dual to large N QCD}},  {\em Nucl.Phys.} {\bf B700} (2004)
  71--88, [\href{http://xxx.lanl.gov/abs/hep-th/0406266}{{\tt
  hep-th/0406266}}].

\bibitem{Abreu:2005uw}
E.~Abreu and P.~Bicudo, {\it {Glueball and hybrid mass and decay with string
  tension below Casimir scaling}},  {\em J.Phys.} {\bf G34} (2007) 195207,
  [\href{http://xxx.lanl.gov/abs/hep-ph/0508281}{{\tt hep-ph/0508281}}].

\bibitem{Brau:2004xw}
F.~Brau and C.~Semay, {\it {Semirelativistic potential model for glueball
  states}},  {\em Phys.Rev.} {\bf D70} (2004) 014017,
  [\href{http://xxx.lanl.gov/abs/hep-ph/0412173}{{\tt hep-ph/0412173}}].

\bibitem{Mathieu:2005wc}
V.~Mathieu, C.~Semay, and F.~Brau, {\it {Casimir scaling, glueballs and hybrid
  gluelumps}},  {\em Eur.Phys.J.} {\bf A27} (2006) 225--230,
  [\href{http://xxx.lanl.gov/abs/hep-ph/0511210}{{\tt hep-ph/0511210}}].

\bibitem{Simonov:2006re}
Y.~Simonov, {\it {Glueballs, gluerings and gluestars in the d=2+1 SU(N) gauge
  theory}},  {\em Phys.Atom.Nucl.} {\bf 70} (2007) 44--52,
  [\href{http://xxx.lanl.gov/abs/hep-ph/0603148}{{\tt hep-ph/0603148}}].

\bibitem{Mathieu:2006bp}
V.~Mathieu, C.~Semay, and B.~Silvestre-Brac, {\it {Semirelativistic potential
  model for low-lying three-gluon glueballs}},  {\em Phys.Rev.} {\bf D74}
  (2006) 054002, [\href{http://xxx.lanl.gov/abs/hep-ph/0605205}{{\tt
  hep-ph/0605205}}].

\bibitem{BoschiFilho:2002vd}
H.~Boschi-Filho and N.~R. Braga, {\it {Gauge / string duality and scalar
  glueball mass ratios}},  {\em JHEP} {\bf 0305} (2003) 009,
  [\href{http://xxx.lanl.gov/abs/hep-th/0212207}{{\tt hep-th/0212207}}].


\bibitem{Polchinski:Vol1}
J.~Polchinski, {\it {String theory. Vol. 1: An introduction to the bosonic
  string}}, .

 
\bibitem{Polchinski:1991ax}
J.~Polchinski and A.~Strominger, {\it {Effective string theory}},  {\em
  Phys.Rev.Lett.} {\bf 67} (1991) 1681--1684.

\bibitem{Aharony:2009gg}
O.~Aharony and E.~Karzbrun, {\it {On the effective action of confining
  strings}},  {\em JHEP} {\bf 0906} (2009) 012,
  [\href{http://xxx.lanl.gov/abs/0903.1927}{{\tt arXiv:0903.1927}}].

\bibitem{ASY}
O.~Aharony, J.~Sonnenschein, and S.~Yankielowicz, {\it {On the quantization of
  rotating open strings with massive endpoints [In preparation]}}, .

\bibitem{Kinar:1998vq}
Y.~Kinar, E.~Schreiber, and J.~Sonnenschein, {\it {Q anti-Q potential from
  strings in curved space-time: Classical results}},  {\em Nucl.Phys.} {\bf
  B566} (2000) 103--125, [\href{http://xxx.lanl.gov/abs/hep-th/9811192}{{\tt
  hep-th/9811192}}].

%\cite{Frolov:2002av}
\bibitem{Frolov:2002av}
  S.~Frolov and A.~A.~Tseytlin,
  ``Semiclassical quantization of rotating superstring in AdS(5) x S**5,''
  JHEP {\bf 0206}, 007 (2002)
  doi:10.1088/1126-6708/2002/06/007
  [hep-th/0204226].
  %%CITATION = doi:10.1088/1126-6708/2002/06/007;%%
  %535 citations counted in INSPIRE as of 27 Jan 2016

\bibitem{Bigazzi:2004ze}
F.~Bigazzi, A.~Cotrone, L.~Martucci, and L.~Pando~Zayas, {\it {Wilson loop,
  Regge trajectory and hadron masses in a Yang-Mills theory from semiclassical
  strings}},  {\em Phys.Rev.} {\bf D71} (2005) 066002,
  [\href{http://xxx.lanl.gov/abs/hep-th/0409205}{{\tt hep-th/0409205}}].

\bibitem{Bali:2000un}
G.~S. Bali, {\it {Casimir scaling of SU(3) static potentials}},  {\em
  Phys.Rev.} {\bf D62} (2000) 114503,
  [\href{http://xxx.lanl.gov/abs/hep-lat/0006022}{{\tt hep-lat/0006022}}].

\bibitem{Armoni:2006ri}
A.~Armoni and B.~Lucini, {\it {Universality of k-string tensions from
  holography and the lattice}},  {\em JHEP} {\bf 06} (2006) 036,
  [\href{http://xxx.lanl.gov/abs/hep-th/0604055}{{\tt hep-th/0604055}}].

\bibitem{Donnachie:1984xq}
A.~Donnachie and P.~Landshoff, {\it {Elastic Scattering and Diffraction
  Dissociation}},  {\em Nucl.Phys.} {\bf B244} (1984) 322.

\bibitem{Isgur:1984bm}
N.~Isgur and J.~E. Paton, {\it {A Flux Tube Model for Hadrons in QCD}},  {\em
  Phys.Rev.} {\bf D31} (1985) 2910.

\bibitem{Meyer:2004jc}
H.~B. Meyer and M.~J. Teper, {\it {Glueball Regge trajectories and the pomeron:
  A Lattice study}},  {\em Phys.Lett.} {\bf B605} (2005) 344--354,
  [\href{http://xxx.lanl.gov/abs/hep-ph/0409183}{{\tt hep-ph/0409183}}].

\bibitem{Meyer:2004gx}
H.~B. Meyer, {\it {Glueball regge trajectories}},
  \href{http://xxx.lanl.gov/abs/hep-lat/0508002}{{\tt hep-lat/0508002}}.

\bibitem{Burden:1982zb}
C.~Burden and L.~Tassie, {\it {Rotating Strings, Glueballs and Exotic Mesons}},
   {\em Austral.J.Phys.} {\bf 35} (1982) 223--233.

\bibitem{Cotrone:2005fr}
A.~L. Cotrone, L.~Martucci, and W.~Troost, {\it {String splitting and strong
  coupling meson decay}},  {\em Phys. Rev. Lett.} {\bf 96} (2006) 141601,
  [\href{http://xxx.lanl.gov/abs/hep-th/0511045}{{\tt hep-th/0511045}}].

\bibitem{Bigazzi:2006jt}
F.~Bigazzi and A.~L. Cotrone, {\it {New predictions on meson decays from string
  splitting}},  {\em JHEP} {\bf 11} (2006) 066,
  [\href{http://xxx.lanl.gov/abs/hep-th/0606059}{{\tt hep-th/0606059}}].

\bibitem{Hashimoto:2007ze}
K.~Hashimoto, C.-I. Tan, and S.~Terashima, {\it {Glueball decay in holographic
  QCD}},  {\em Phys. Rev.} {\bf D77} (2008) 086001,
  [\href{http://xxx.lanl.gov/abs/0709.2208}{{\tt arXiv:0709.2208}}].

\bibitem{Brunner:2015oqa}
F.~Br{\"u}nner, D.~Parganlija, and A.~Rebhan, {\it {Glueball Decay Rates in the
  Witten-Sakai-Sugimoto Model}},  {\em Phys. Rev.} {\bf D91} (2015), no.~10
  106002, [\href{http://xxx.lanl.gov/abs/1501.0790}{{\tt arXiv:1501.0790}}].

\bibitem{Brunner:2015yha}
F.~Br{\"u}nner and A.~Rebhan, {\it {Nonchiral enhancement of scalar glueball
  decay in the Witten-Sakai-Sugimoto model}},
  \href{http://xxx.lanl.gov/abs/1504.0581}{{\tt arXiv:1504.0581}}.

\bibitem{Crede:2008vw}
V.~Crede and C.~Meyer, {\it {The Experimental Status of Glueballs}},  {\em
  Prog.Part.Nucl.Phys.} {\bf 63} (2009) 74--116,
  [\href{http://xxx.lanl.gov/abs/0812.0600}{{\tt arXiv:0812.0600}}].

\bibitem{PDG:2014}
{\bf Particle Data Group} Collaboration, K.~Olive et~al., {\it {Review of
  Particle Physics}},  {\em Chin.Phys.} {\bf C38} (2014) 090001.

\bibitem{Klempt:2007cp}
E.~Klempt and A.~Zaitsev, {\it {Glueballs, Hybrids, Multiquarks. Experimental
  facts versus QCD inspired concepts}},  {\em Phys.Rept.} {\bf 454} (2007)
  1--202, [\href{http://xxx.lanl.gov/abs/0708.4016}{{\tt arXiv:0708.4016}}].

\bibitem{Mathieu:2008me}
V.~Mathieu, N.~Kochelev, and V.~Vento, {\it {The Physics of Glueballs}},  {\em
  Int.J.Mod.Phys.} {\bf E18} (2009) 1--49,
  [\href{http://xxx.lanl.gov/abs/0810.4453}{{\tt arXiv:0810.4453}}].

\bibitem{Ochs:2013gi}
W.~Ochs, {\it {The Status of Glueballs}},  {\em J.Phys.} {\bf G40} (2013)
  043001, [\href{http://xxx.lanl.gov/abs/1301.5183}{{\tt arXiv:1301.5183}}].

\bibitem{Nebreda:2011cp}
J.~Nebreda, J.~Pelaez, and G.~Rios, {\it {Enhanced non-quark-antiquark and
  non-glueball Nc behavior of light scalar mesons}},  {\em Phys.Rev.} {\bf D84}
  (2011) 074003, [\href{http://xxx.lanl.gov/abs/1107.4200}{{\tt
  arXiv:1107.4200}}].

\bibitem{Anisovich:2002us}
V.~Anisovich, {\it {Systematics of quark anti-quark states and scalar exotic
  mesons}},  {\em Phys.Usp.} {\bf 47} (2004) 45--67,
  [\href{http://xxx.lanl.gov/abs/hep-ph/0208123}{{\tt hep-ph/0208123}}].

\bibitem{Masjuan:2012gc}
P.~Masjuan, E.~Ruiz~Arriola, and W.~Broniowski, {\it {Systematics of radial and
  angular-momentum Regge trajectories of light non-strange
  $q\overline{q}$-states}},  {\em Phys.Rev.} {\bf D85} (2012) 094006,
  [\href{http://xxx.lanl.gov/abs/1203.4782}{{\tt arXiv:1203.4782}}].

\bibitem{Bugg:2012yt}
D.~Bugg, {\it {Comment on “Systematics of radial and angular-momentum Regge
  trajectories of light nonstrange $q\overline{q}$-states”}},  {\em
  Phys.Rev.} {\bf D87} (2013), no.~11 118501,
  [\href{http://xxx.lanl.gov/abs/1209.3481}{{\tt arXiv:1209.3481}}].

\bibitem{Ablikim:2012ft}
{\bf BESIII} Collaboration, M.~Ablikim et~al., {\it {Study of the
  near-threshold ωϕ mass enhancement in doubly OZI-suppressed J/ψ→γωϕ
  decays}},  {\em Phys.Rev.} {\bf D87} (2013), no.~3 032008,
  [\href{http://xxx.lanl.gov/abs/1211.5668}{{\tt arXiv:1211.5668}}].

\bibitem{Bai:1996wm}
{\bf BES Collaboration} Collaboration, J.~Bai et~al., {\it {Studies of xi
  (2230) in J / psi radiative decays}},  {\em Phys.Rev.Lett.} {\bf 76} (1996)
  3502--3505.

\bibitem{Benslama:2002pa}
{\bf CLEO} Collaboration, K.~Benslama et~al., {\it {Anti-search for the
  glueball candidate f(J)(2220) in two -photon interactions}},  {\em Phys.Rev.}
  {\bf D66} (2002) 077101, [\href{http://xxx.lanl.gov/abs/hep-ex/0204019}{{\tt
  hep-ex/0204019}}].

\bibitem{Vladimirsky:2001ek}
V.~Vladimirsky, V.~Grigorev, O.~Erofeeva, Y.~Katinov, V.~Lisin, et~al., {\it
  {Resonance maximum in the system of two K(S) mesons at 1450-MeV}},  {\em
  Phys.Atom.Nucl.} {\bf 64} (2001) 1895--1897.

\bibitem{Vijande:2004he}
J.~Vijande, F.~Fernandez, and A.~Valcarce, {\it {Constituent quark model study
  of the meson spectra}},  {\em J.Phys.} {\bf G31} (2005) 481,
  [\href{http://xxx.lanl.gov/abs/hep-ph/0411299}{{\tt hep-ph/0411299}}].

\bibitem{Athenodorou:2010cs}
A.~Athenodorou, B.~Bringoltz, and M.~Teper, {\it {Closed flux tubes and their
  string description in D=3+1 SU(N) gauge theories}},  {\em JHEP} {\bf 02}
  (2011) 030, [\href{http://xxx.lanl.gov/abs/1007.4720}{{\tt
  arXiv:1007.4720}}].

\bibitem{Bochicchio:2013aha}
M.~Bochicchio, {\it {Yang-Mills mass gap, Floer homology, glueball spectrum,
  and conformal window in large-N QCD}},
  \href{http://xxx.lanl.gov/abs/1312.1350}{{\tt arXiv:1312.1350}}.

\bibitem{Bochicchio:2013sra}
M.~Bochicchio, {\it {Glueball and meson spectrum in large-N massless QCD}},
  \href{http://xxx.lanl.gov/abs/1308.2925}{{\tt arXiv:1308.2925}}.

\bibitem{Caselle:2015tza}
M.~Caselle, A.~Nada, and M.~Panero, {\it {Hagedorn spectrum and thermodynamics
  of SU(2) and SU(3) Yang-Mills theories}},
  \href{http://xxx.lanl.gov/abs/1505.0110}{{\tt arXiv:1505.0110}}.

\bibitem{Gregory:2012hu}
E.~Gregory, A.~Irving, B.~Lucini, C.~McNeile, A.~Rago, et~al., {\it {Towards
  the glueball spectrum from unquenched lattice QCD}},  {\em JHEP} {\bf 1210}
  (2012) 170, [\href{http://xxx.lanl.gov/abs/1208.1858}{{\tt
  arXiv:1208.1858}}].

\bibitem{Albanese:1987ds}
{\bf APE} Collaboration, M.~Albanese et~al., {\it {Glueball Masses and String
  Tension in Lattice QCD}},  {\em Phys.Lett.} {\bf B192} (1987) 163--169.

\bibitem{Morningstar:1999rf}
C.~J. Morningstar and M.~J. Peardon, {\it {The Glueball spectrum from an
  anisotropic lattice study}},  {\em Phys.Rev.} {\bf D60} (1999) 034509,
  [\href{http://xxx.lanl.gov/abs/hep-lat/9901004}{{\tt hep-lat/9901004}}].

\bibitem{Chen:2005mg}
Y.~Chen, A.~Alexandru, S.~Dong, T.~Draper, I.~Horvath, et~al., {\it {Glueball
  spectrum and matrix elements on anisotropic lattices}},  {\em Phys.Rev.} {\bf
  D73} (2006) 014516, [\href{http://xxx.lanl.gov/abs/hep-lat/0510074}{{\tt
  hep-lat/0510074}}].

\bibitem{Bali:1993fb}
{\bf UKQCD Collaboration} Collaboration, G.~Bali et~al., {\it {A Comprehensive
  lattice study of SU(3) glueballs}},  {\em Phys.Lett.} {\bf B309} (1993)
  378--384, [\href{http://xxx.lanl.gov/abs/hep-lat/9304012}{{\tt
  hep-lat/9304012}}].

\bibitem{Lucini:2014paa}
B.~Lucini, {\it {Glueballs from the Lattice}},  {\em PoS} {\bf QCD-TNT-III}
  (2013) 023, [\href{http://xxx.lanl.gov/abs/1401.1494}{{\tt
  arXiv:1401.1494}}].

\bibitem{Lucini:2004my}
B.~Lucini, M.~Teper, and U.~Wenger, {\it {Glueballs and k-strings in SU(N)
  gauge theories: Calculations with improved operators}},  {\em JHEP} {\bf
  0406} (2004) 012, [\href{http://xxx.lanl.gov/abs/hep-lat/0404008}{{\tt
  hep-lat/0404008}}].

\bibitem{Ganor:1994rm}
O.~Ganor, J.~Sonnenschein, and S.~Yankielowicz, {\it {Folds in 2-D string
  theories}},  {\em Nucl.Phys.} {\bf B427} (1994) 203--244,
  [\href{http://xxx.lanl.gov/abs/hep-th/9404149}{{\tt hep-th/9404149}}].

%\cite{Dubovsky:2015zey}
\bibitem{Dubovsky:2015zey}
  S.~Dubovsky and V.~Gorbenko,
  ``Towards a Theory of the QCD String,''
  arXiv:1511.01908 [hep-th].
  %%CITATION = ARXIV:1511.01908;%%
  %1 citations counted in INSPIRE as of 15 Jan 2016

  %\cite{Lambiase:1995st}
\bibitem{Lambiase:1995st}
  G.~Lambiase and V.~V.~Nesterenko,
  ``Quark mass correction to the string potential,''
  Phys.\ Rev.\ D {\bf 54}, 6387 (1996)
  doi:10.1103/PhysRevD.54.6387
  [hep-th/9510221].
  %%CITATION = doi:10.1103/PhysRevD.54.6387;%%
  %22 citations counted in INSPIRE as of 16 Jan 2016

%\cite{Shuryak:2013sra}
\bibitem{Shuryak:2013sra}
  E.~Shuryak and I.~Zahed,
  ``New regimes of the stringy (holographic) Pomeron and high-multiplicity $pp$ and $pA$ collisions,''
  Phys.\ Rev.\ D {\bf 89}, no. 9, 094001 (2014)
  doi:10.1103/PhysRevD.89.094001
  [arXiv:1311.0836 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevD.89.094001;%%
  %22 citations counted in INSPIRE as of 28 Jan 2016


\end{thebibliography}\endgroup




